Improving the Faithfulness of Abstractive Summarization via Entity Coverage Control

Abstractive summarization systems leveraging pre-training language models have achieved superior results on benchmark datasets. However, such models have been shown to be more prone to hallucinate facts that are unfaithful to the input context. In this paper, we propose a method to remedy entity-level extrinsic hallucinations with Entity Coverage Control (ECC). We first compute entity coverage precision and prepend the corresponding control code for each training example, which implicitly guides the model to recognize faithfulness contents in the training phase. We further extend our method via intermediate fine-tuning on large but noisy data extracted from Wikipedia to unlock zero-shot summarization. We show that the proposed method leads to more faithful and salient abstractive summarization in supervised fine-tuning and zero-shot settings according to our experimental results on three benchmark datasets XSum, Pubmed, and SAMSum of very different domains and styles.

==> source/TODO.tex <==
\section{TODO -- Remaining Items}
\begin{itemize}
    \item \answerTODO{get Semih's v2 human evaluation results}
    \item \answerTODO{collect the numbers and fill the table}

\end{itemize}


\subsection{Meeting -- 09/13/21}
\begin{itemize}
    \item We need to rewrite the paper in a stronger fashion
    \item Abstract + Intro should motivate the problem and our solution in a stronger way
    \item Method part should be written in a more generic way (generally applicable) -- 
    \item Method part should include more details and emphasize the novelty ...
    \item Analysis part can be extended by further intuition
    \item Analysis -- The effect of entity-level control on more general faithfulness such as ngram-based faithfulness?
    \item ...

\end{itemize}




==> source/approach.tex <==
\section{Methods}
\begin{figure}
    \centering
    \includegraphics[width = 0.5\textwidth]{figures/wiki_model.png}
    \caption{ The Overall Training Pipeline of Our Proposed Method. \wojciech{This figure could use some work. It's hard to understand from the caption and lables in the figure what is happening. Is this an overall pipeline? Is it specific to the entity method? Maybe try to include both cases in the figure?}}
    \label{wiki_figure}
\end{figure}
In this section, we introduce our proposed methods in great detail. We first present how to address entity hallucination in the supervised setting, and then show how to extend it\wojciech{extend the framework?} to a controllable intermediate pre-training model \wojciech{controllable intermediate pre-training scheme/strategy} in the zero-shot setting.

\subsection{Entity Control for Hallucination}
Following \cite{nan-etal-2021-entity}, we first quantify the degree of entity-level hallucination with entity coverage precision $\mathbf{prec_{en}}$. It measures the percentage of named entities in the summary covered in the source document, which could be defined as \wojciech{which is defined as/defined as:}:

\begin{equation}
    \mathbf{prec_{en}} = \mathcal{N}(h \cap s)/\mathcal{N}(h), 
\end{equation}
where $\mathcal{N}(h)$ and $\mathcal{N}(h \cap s)$ represent the number of named-entities in the hypothesis (generated summary) and named-entities in both the generated summary and the source document.

To enable the model to learn different entity level faithfulness patterns, we use entity coverage precision $\mathbf{prec_{en}}$ as a pseudo label in the training phase. We first compute $\mathbf{prec_{en}}$ for each training document and reference summary pair in advance. Then, we quantize $\mathbf{prec_{en}}$ into $k$ discrete bins, each representing a range of entity faithfulness. These bin boundaries are selected to make sure that each bin contains roughly the same number of training examples to avoid data imbalance. We then represent each bin by a special token ${S_i}$ and add all special tokens $\{S_1, S_2, . . . , S_k\}$ to the input vocabulary of our backbone pre-trained language model (BART) \cite{lewis-etal-2020-bart}. 

During training, we prepend the corresponding pseudo label ${S_i}$ to the input document as control code. In this way, the summary generation is conditioned on both the source document and its control code ${S_i}$. Then during inference, we prepend the high faithfulness special token ${S_k}$ to all documents in the test set and generate faithful summaries.
\wojciech{We write what we do, but we don't write why. Maybe mention somehwere in this section what the intuition here is?}

\subsection{Controllable Intermediate Pre-training with Wikipedia}

Large sized \wojciech{large scale? }pre-trained language models such as BERT \cite{devlin2018bert} and BART \cite{lewis2019bart} perform poorly in the zero-shot setting \wojciech{in which zero-shot setting?} since sentence salience information is not learned through their pre-training tasks. Thus, we propose an controllable generalized intermediate pre-training using unsupervised Wikipedia data for zero-shot summarization. The overall training pipeline is shown in Fig~\ref{wiki_figure}.

Following Wikitransfer \cite{fabbri-etal-2021-improving}, we first generate domain-specific intermediate data from Wikipedia articles. For each downstream target dataset, we generate pseudo document and summary pairs with the same average document $n$ and summary $m$ length and the same abstractiveness level $a$. Here abstraciveness level is defined as the upper bound extractive
ROUGE1 \cite{lin2004rouge} performance of the target dataset. For each available Wikipedia articles in a Wikipedia dump, we use the first
$m$ sentences of the Wikipedia article as
a pseudo summary and the following $n$ sentences as a pseudo source document. We only keep examples that has similar extractive oracle $a$. In this way, we could gather a domain-specific train set that contains pseudo document summary pairs with similar characteristics to the target dataset.

Instead of training different models for different downstream task datasets as in WikiTransfer \cite{fabbri-etal-2021-improving}, we propose a unified model that generalizes well across target datasets in different domains in the zero-shot setting. For each domain-specific training subset, we give it another special token ${D_j}$ as a pseudo label to represent the domain information and also add all these special tokens $\{D_1, D_2, . . . , D_l\}$ to the input vocabulary of BART. 

In the training phase, we preprend the corresponding domain label ${D_j}$ to the intermediate document, and we could control the domain of generated summaries by prepending different domain labels during inference. We could also stack the domain-specific pseudo labels with entity faithfulness pseudo labels together as shown in Fig ~\ref{wiki_figure} for faithful zero-shot summarization. 
\wojciech{Similar comment to last subsection. We mention how, but ommit the why. Maybe motivate this idea a bit?}
